Global Graph Counterfactual Explanation: A Subgraph Mapping Approach

Graph Neural Networks (GNNs) have been widely deployed in various real-world applications. However, most GNNs are black-box models that lack explanations. One strategy to explain GNNs is through counterfactual explanation, which aims to find minimum perturbations on input graphs that change the GNN predictions. Existing works on GNN counterfactual explanations primarily concentrate on the local-level perspective (i.e., generating counterfactuals for each individual graph), which suffers from information overload and lacks insights into the broader cross-graph relationships. To address such issues, we propose GlobalGCE, a novel global-level graph counterfactual explanation method. GlobalGCE aims to identify a collection of subgraph mapping rules as counterfactual explanations for the target GNN. According to these rules, substituting certain significant subgraphs with their counterfactual subgraphs will change the GNN prediction to the desired class for most graphs (i.e., maximum coverage). Methodologically, we design a significant subgraph generator and a counterfactual subgraph autoencoder in our GlobalGCE, where the subgraphs and the rules can be effectively generated. Extensive experiments demonstrate the superiority of our GlobalGCE compared to existing baselines. Our code can be found at https://anonymous.4open.science/r/GlobalGCE-92E8.

==> Sections/2-Preliminaries.tex <==
\vspace{-0.1in}
\section{Preliminaries and Related Work}\label{sec:preliminaries}
In this section, we provide background information on the local-level GNN explainer and the only known global-level GNN explainer GCFExplainer~\citep{huang2023global}, both of which are necessary for understanding our GlobalGCE. Please refer to the Appendix for more details.

\subsection{Local Counterfactual Explainers for GNN}\label{subsec:local_gnn_explainer}
% What is the necessary information about GlobalGCE from the LCE4G that we want the audience to know? 
% In the GCFExplainer paper, they give (1) the definition of the problem, e.g., what is the graph, what is the classifier like, what is a counterfactual explanation; 
% The existing counterfactual explanation methods take a local perspective. Specifically, they ...
% they introduce the distance they adopt, do we need to do that?

Let $G = (\boldsymbol{X}, \boldsymbol{\boldsymbol{A}}, \boldsymbol{E})$ denote a graph with $n$ nodes, where $\boldsymbol{A} \in \{0,1\}^{n \times n}$ is the graph adjacency matrix, $\boldsymbol{X}\in \mathbb{R}^{n\times l}$ is the node attribute matrix ($l$ is the node attribute size), $\boldsymbol{E}\in \mathbb{R}^{(n(n-1)/2)\times m}$ is the edge attribute matrix ($(n(n-1)/2)$ is the number of all possible edges, $m$ is the edge attribute size). We denote $\phi:\mathcal{G}\rightarrow \mathcal{Y}$ as a GNN, where $\mathcal{G}$ is the input graph space, $\mathcal{Y}=\{0,1\}$ is the label space (for simplicity, $0$ represents the undesired class, $1$ represents the desired class). We treat the GNN as a black-box model, where only the output label $y \in \mathcal{Y}$ produced by the model in response to an input graph $G \in \mathcal{G}$, is accessible.

Most existing GCE works are restricted to the local level~\citep{prado2023survey, ying2019gnnexplainer, bajaj2021robust, lucic2022cf, ma2022clear, tan2022learning}, where the explainer aims to learn a function $f: \mathcal{G} \rightarrow \mathcal{G}$ that maps each individual undesired input graph $G$ (e.g., $\phi(G)=0$) to its counterfactual $G^{cf}=f(G)$ (e.g., $\phi(G^{cf})=1$). Since the exact counterfactual, which is usually defined as the graph with the desired label that has the smallest perturbation from the original graph, is \emph{intractable} to identify due to the combinatorial complexity, current literature typically relaxes the definition of the counterfactual $G^{cf}$ as a desired graph within a graph distance threshold $\theta$ from $G$. However, as discussed before, local-level counterfactual explainers fail to offer global insights and have information overload problems. Next, we introduce GCFExplainer~\citep{huang2023global}, the only known global counterfactual explainer for GNNs which, although having certain limitations, provides a high-level summary for GNN behavior on the input graph dataset.

\subsection{Global Counterfactual Explainers}\label{subsec: global_gnn_explainer}
Global counterfactual explanation (CE) is attracting more attention~\citep{rawal2020beyond,ley2022global,ley2022diverse, kanamori2022counterfactual}. Among them, AReS formulates the global CE as finding a set of triples $\mathcal{R}=\{(q_i, c_i, c_i')\}_{i=1}^{t}$. Here, each triple is a CE rule: for a sample satisfying condition $q_i$, its counterfactual can be acquired by changing the feature $c_i$ to $c_i'$. Despite insightful, AReS is computationally expensive because AReS selects CE rules from the set of all combinations of conditions ($q$s) and sample features ($c$s). \citet{ley2022global} solve the problem by a fast rule evaluator as a preprocessor of ARes to filter out the less-likely CE rules. Since using triples to represent global counterfactuals does not fit continuous sample features, 
 GLOBE-CE~\citep{ley2023globe} formulate the global CE as a translation of the sample features with fixed direction and varied magnitude. However, those models are tailored for i.i.d. datasets and non-trivial to be adapted to graph datasets. 
 
\citet{huang2023global} propose the only known global counterfactual explainer for graphs: GCFExplainer. For an input graph dataset $\mathcal{G}$ ($|\mathcal{G}|=n$), GCFExplainer aims to find a small set of counterfactuals $\mathcal{C}$ ($|\mathcal{C}|=k\ll n$) that can cover the most input graphs within a graph distance threshold $\theta$. Here, a counterfactual $G_i^{cf}\in\mathcal{C}$ covers a graph $G_i$ if the distance between the graph $G_i$ and $G_i^{cf}$ is smaller than $\theta$.
% The authors first adopt the vertex-reinforced random walk (VRRW) model to generate the counterfactual set $\mathcal{C}$. Specifically, they first build a meta-graph where each node of the meta-graph represents a graph in the domain of $\mathcal{G}$. Therefore, the meta-graph contains $\mathcal{G}$ and all their possible counterfactuals. Then, they add edges for node pairs in the meta-graph, i.e., the graphs in $\mathcal{G}$, with a graph edit distance of one. In this meta-graph, a vertex-reinforced random walk is performed. ``Vertex-reinforced'' means that the transition probability at each step of the walk is inversely proportional to the frequency of visits to neighboring nodes. This ensures a diverse exploration of nodes (input graphs) in the meta-graph, preventing the walk from being confined to a limited set of nodes. They collect the footprint nodes that are identified by the GNN $\phi$ as desired graphs, thus forming set of $\mathcal{C}$. 
However, GCFExplainer exhibits some limitations, as discussed in earlier. Differently, our work formulates the global GCE as a small set of \emph{counterfactaul subgraph mappings} (CSM), where each CSM is in the form of $\{g\rightarrow g^{cf}\}$.
% where the graph distance between $g$ and $g^{cf}$ is smaller or equal to $\theta$.
Here, $g\subseteq G$ for some $G\in \mathcal{G}$, and $g^{cf}$ is called the \emph{counterfactual subgraph} of $g$. With a budget for CSMs, our goal is to identify those CSMs which, upon editing a subgraph of the input graph into its counterfactual subgraph, result in the highest proportion of graphs in $\mathcal{G}$ achieving their counterfactuals. 

% For an undesired input graph $G$ containing $g$, editing the $g$ in $G$ to $g^{cf}$ will likely change $G$ to its counterfactual $G^{cf}$. We call this modification process as ``applying subgraph mapping $\{g\rightarrow g^{cf}\}$ to $G$''.

% why do we want to briefly summarize that paper? what thing do you want from the paper, we need something directly from that paper that can offer some insights. Basically, we need the things that can be directly used in our case but not talking about other people's work. 


% In this study, we employ a graph prediction model, symbolized as $f: \mathbf{G} \rightarrow \mathbf{Y}$, which maps graphs $G$ to their corresponding labels in $Y$. We make the assumption that $f$ operates as a Graph Neural Network (GNN) classifier. For an arbitrary graph $G \in \mathbf{G}$, its counterfactual counterpart, $G^{CF}$, is postulated to bear a high degree of resemblance to the original graph $G$. However, the label $Y^{CF}$ ascribed to $G^{CF}$ is intended to align with the target label $Y^*$.
% The counterfactual explanation, as an important concept in causal inference~\citep{pearl2009causality}, is defined based on a causal model~\citep{kusner2017counterfactual}:
% \begin{definition}\label{def:causal_model}
%   (Causal Model) A causal model is a triple of sets ($U, V, F$): $U$ is the set of latent background variables (exogenous variables) that are not caused by any variable in $V$, and $V$ is the set of observable variables (endogenous variables). $F$ is the set of functions $\{f_1, ..., f_n\}$, called structural equations, such that $V_i = f_i(pa_i, U_{i})$, where $pa_i \subset V\setminus\{V_i\}$ is the ``parents'' of $V_i$, and $U_{i} \subset U$.
% \end{definition}
% Given a causal model $(U, V, F)$ and evidence $W=w$, we call $Z \leftarrow z$, the change of observable variables set $Z$ to $z$, as a counterfactual explanation of the causal model w.r.t. $Y$, if $(Y_{Z\leftarrow z}(U)|W=w)$ is not equal to $(Y_{Z}(U)|W=w)$. Here $(Y_{Z}(U)|W=w)$ is the result of $Y$ if we are given the observable variables set $Z \subset V$ determined by the structural equations, background variables $U$, and evidence $W=w$. Analogously, with the same background variables $U$ and evidence $W=w$, $(Y_{Z\leftarrow z}(U)|W=w)$ is the result of $Y$ if observable variables set $Z$ is changed to $z$. Typically, we require $Z \leftarrow z$ to be the smallest change such that $(Y_{Z}(U)|W=w)$ is not equal to $(Y_{Z\leftarrow z}(U)|W=w)$, and the $(Y_{Z}(U)|W=w)$ is considered as some undesired result, $(Y_{Z\leftarrow z}(U)|W=w)$ is the desired result. Now, we consider the scenario of the graph classification task, where the input graph $G=(A, X)$ and GNN model prediction $Y^{\phi}$ are observable variables. The counterfactual explanation of the causal model $(U, V=(G,Y^{\phi}), F)$ w.r.t. $Y^{\phi}$ is to find the change $G=(A, X) \leftarrow \hat{G}=(\hat{A},\hat{X})$ such that the undesired result $(Y^{\phi}_{Z=G}|W=w)$ is changed to the desired result $(Y^{\phi}_{z=\hat{G}}|W=w)$. 
% As previously delineated, extant methodologies in the domain of graph counterfactual explanations predominantly exhibit limitations in terms of global interpretability and are susceptible to issues related to information overload~\cite{abrate2021counterfactual, bajaj2021robust, guidotti2019factual,huang2023global, lucic2022cf, prado2022survey}. To furnish additional context, we turn our attention to GCFExplainer, the sole framework in the literature that addresses global graph counterfactual explanations~\cite{huang2023global}. Within the scope of their investigation, the authors articulate the concept of global counterfactual explanation in the context of graph classification as follows:





% \begin{definition}\label{def:interpretable_cfe}
% (Interpretability in CFE) For a graph space $\mathbf{G}$ in certain domain, a interpretable counterfactual explanation for $\mathbf{G}$ is a graph counterfactual explanation set $S=(G_i,\tilde{G}_i)_{i=1}^{n}$ satisfying
% \begin{itemize}
%   \item For any $G\in \mathbf{G}$, there is at least a $(G_i,\tilde{G_i})$ such that $G_i$ is a subgraph of $G$.
%   \item By applying $(G_i,\tilde{G_i})$ to subgraph of $G$ produces the counterfactul of $G$.
% \end{itemize}
% \end{definition}



==> Sections/8-Disclaimer.tex <==
\section{Disclaimer}
This paper was prepared for informational purposes “in part” by the CDAO group of JPMorgan Chase & Co and its affiliates (“J.P. Morgan”) and is not a product of the Research Department of J.P. Morgan. J.P. Morgan makes no representation and warranty whatsoever and disclaims all liability, for the completeness, accuracy or reliability of the information contained herein. This document is not intended as investment research or investment advice, or a recommendation, offer or solicitation for the purchase or sale of any security, financial instrument, financial product or service, or to be used in any way for evaluating the merits of participating in any transaction, and shall not constitute a solicitation under any jurisdiction or to any person, if such solicitation under such jurisdiction or to such person would be unlawful.
